Contributions to Representation Learning with Graph Autoencoders and Applications to Music Recommendation

Graph autoencoders (GAE) and variational graph autoencoders (VGAE) emerged as two powerful groups of unsupervised node embedding methods, with various applications to graph-based machine learning problems such as link prediction and community detection. Nonetheless, at the beginning of this Ph.D. project, GAE and VGAE models were also suffering from key limitations, preventing them from being adopted in the industry. In this thesis, we present several contributions to improve these models, with the general aim of facilitating their use to address industrial-level problems involving graph representations. Firstly, we propose two strategies to overcome the scalability issues of previous GAE and VGAE models, permitting to effectively train these models on large graphs with millions of nodes and edges. These strategies leverage graph degeneracy and stochastic subgraph decoding techniques, respectively. Besides, we introduce Gravity-Inspired GAE and VGAE, providing the first extensions of these models for directed graphs, that are ubiquitous in industrial applications. We also consider extensions of GAE and VGAE models for dynamic graphs. Furthermore, we argue that GAE and VGAE models are often unnecessarily complex, and we propose to simplify them by leveraging linear encoders. Lastly, we introduce Modularity-Aware GAE and VGAE to improve community detection on graphs, while jointly preserving good performances on link prediction. In the last part of this thesis, we evaluate our methods on several graphs extracted from the music streaming service Deezer. We put the emphasis on graph-based music recommendation problems. In particular, we show that our methods can improve the detection of communities of similar musical items to recommend to users, that they can effectively rank similar artists in a cold start setting, and that they permit modeling the music genre perception across cultures.

==> frontmatter/acknowledgements.tex <==
\addcontentsline{toc}{section}{Acknowledgments}


First and foremost, I would like to express my deepest gratitude to \textbf{Romain Hennequin} from Deezer, who served as my primary supervisor over the past three years and devoted countless hours to reviewing this thesis, along with all my papers, code, posters, and presentations.  In addition, Romain always supported me in this tumultuous but exciting journey that a PhD program inevitably constitutes. His scientific rigor and his intelligence, combined with his kindness and his availability, make him the perfect mentor. I learned a lot by his side and
I sincerely hope, without really doubting it, that our personal ties will last~long~after~this~thesis.

I would also like to thank \textbf{Michalis Vazirgiannis}, my supervisor on the Polytechnique side, for his guidance and the confidence he has placed in me throughout this PhD. By welcoming me to his team at LIX, he made this thesis possible. His support allowed me to teach at Polytechnique and to collaborate with the talented LIX researchers mentioned in the next paragraphs. I am grateful not only for these opportunities but also for his trust, insightful advice, and perspective, which helped shape the direction of my research.

I am honored to have six world-class external researchers on my defense committee. In particular, \textbf{Patrick Gallinari} from Sorbonne Université and \textbf{Yizhou Sun} from UCLA both accepted to spend time and effort to review this thesis. I would like to thank them for their careful reports and valuable comments. Moreover, I am grateful to \textbf{Thomas Bonald} from Télécom~Paris, who acted as President of this committee and shared his profound expertise on graph learning. I~would also like to thank \textbf{Markus Schedl} from JKU, who traveled from Austria to attend the defense, and \textbf{Jie Tang} from Tsinghua University, who virtually joined us from China. They reinforced this jury by bringing their outstanding knowledge on recommender systems and graph mining, respectively. Last, but not least, I am grateful to \textbf{Michal Valko} from INRIA and DeepMind.~His \textit{``Graphs in Machine Learning''} course at ENS Paris-Saclay, back in 2015, initially
triggered my fascination for graphs. His presence on my committee therefore~means~a~lot~to~me.

Besides, I would like to thank \textbf{Deezer}, where I have been fortunate to work for the past five years, for having entirely funded my PhD project. This would never have been possible without the keen support of \textbf{Aurélien Hérault}, our Chief Data and Research Officer, who defended this project when few people believed in it. I am indebted for the opportunities he offered me.

In particular, when I started this PhD in 2018, I simultaneously joined our \textbf{Deezer Research} team as a researcher, after having worked as a data scientist at Deezer for nearly two years.
Pursuing full-time research in such a team was not something I thought would have been possible \textit{before} getting my PhD degree. Thanks to Deezer Research, I have always conducted my projects in excellent material and intellectual conditions, while being inspired by the numerous research problems arising in the music streaming industry. I am convinced that I have achieved much more in such an environment than I would, had I stayed ``only'' in an academic laboratory. Over the years, I have also seen our team double in size, gain reputation, and start regularly publishing in top-tier conferences and journals. I am proud to have been part of this adventure.

The success of Deezer Research owes a lot to the scientific and human qualities of our Director of Research \textbf{Manuel Moussallam}, who is unanimously recognized as one of the best team leaders of the company. I would like to thank him for his benevolence and his constant support,
as well as for the time and effort he spent reviewing all my papers. I am also glad that we could co-author several of them together over the last three years.

Apart from ``Manu'', I have a special thought for two other researchers from our team. The first one is \textbf{Viet-Anh Tran}, who co-supervised the first year of my PhD before his sabbatical leave, and also co-authored most of the papers I published during my third year. Besides his never-failing encouragement, I strongly benefited from his expertise in recommender systems and his understanding of the related engineering aspects, which were both extremely valuable to carry out our joint projects. The second one is \textbf{Elena V. Epure}. The beginning of my PhD coincided with her own oral defense, where I was impressed by the quality of her work. This
positive impression was confirmed and even reinforced during our fruitful joint project on music genre representations. I would like to thank her for her hard work and dedication, for the time she spent reviewing several of my other papers, and for her friendly support~throughout~these~years.

I would also like to express my gratitude to all the other rock stars I have crossed paths with at Deezer Research, in alphabetical order: \textbf{Darius Afchar}, \textbf{Mickael Arcos}, \textbf{Marion Baranes}, \textbf{Robin Cura}, \textbf{Dorian Desblancs}, \textbf{Karim M. Ibrahim}, \textbf{Anis Khlif}, \textbf{Thomas Louail}, \textbf{Benjamin Martin}, \textbf{Bruno Massoni Sguerra}, \textbf{Kristina Matrosova}, \textbf{Gabriel Meseguer Brocal}, \textbf{Rodolfo Ripado}, \textbf{Jimena Royo-Letelier}, \textbf{Clémence Saillard}, \textbf{Andrea Vaglio} and \textbf{Félix Voituret}. I do not forget my former intern \textbf{Raphaël Ginoulhac}, and the dozen other talented interns from all around the world that our team has~welcomed~in~recent~years.

In addition, I am grateful to my colleagues from other teams at Deezer. While it is impossible for me to cite everyone, be sure that I have a thought for you if we have ever worked, played music, and/or drunk a few beers together. In particular, many thanks to all members of our \textbf{Recommendation team}, led by \textbf{Thomas Bouabça}, and especially to the five people from this team who were involved in the research presented in this thesis: \textbf{Léa Briand} on our system for user cold start recommendation (I also thank her for her constant support throughout these years); \textbf{Mathieu Morlon} on the engineering aspects of this system; \textbf{Théo Bontempelli} on carousel personalization with contextual bandits; \textbf{Walid Bendada} on both of the two aforementioned projects; and of course \textbf{Benjamin Chapus} on all things related to graph-based music recommendation. I also thank all members of the \textbf{Data Analytics team}, my first team at Deezer from 2017 to 2018, and notably \textbf{Clémence Saillard} (wow, you are cited twice!) and \textbf{Sébastien Mammale}. By hiring me five years ago, they became the first ones to trust me at Deezer, which I have not forgotten.

While one can achieve a lot in a great team, one can achieve even more in \textit{two} great teams. I am therefore equally grateful to the \textbf{Data Science and Mining team} of the \textbf{LIX laboratory}.
I sincerely enjoyed every moment I spent in this research group (or, at least, every moment unrelated to the RER B and 91.06 C buses). As, once again, it is hard for me to mention everyone, I address a collective ``thank you'' to all past and current members of this team, and,
in the following, I dedicate a few additional words to those I have been fortunate to work with.

The first name to mention is the one of \textbf{Johannes F. Lutzeyer}, whose help during the last year of my PhD was extremely important and valuable to me. Besides our year-long joint work on community detection, Johannes spent hours reviewing a large part of this thesis with outstanding thoroughness, kindly forwarded me his own thesis template, and also proofread most of my recent papers. I am also thankful for his friendly support, especially over the last few months. Moreover, I would like to thank \textbf{Jean-Baptiste Remy}. I keep an excellent memory of
our weekly discussions during the first half of my PhD, when the lab was often still empty, and on various topics ranging from science to rugby, and from my (totally fine) coffee consumption to life in academia. I would also like to thank him for his help on
the FastGAE paper and his dedication during our common teaching activities.

In addition, I would like to express my gratitude to \textbf{George Dasoulas}, for our recent joint work on community detection, but also for our numerous discussions throughout these years (the~key~steps~of~our respective PhD programs often happened at the same time); to \textbf{Stratis Limnios}, for our collaboration on gravity-inspired graph autoencoders, and our exchanges since my internship at LIX in 2016; to \textbf{Giannis Nikolentzos}, for the time and effort he spent reviewing the first part of this thesis; to \textbf{Jesse Read}, for his precious help when we needed to prepare our common teaching activities; to \textbf{Nikolaos Tziortziotis}, for his guidance during our joint work on adaptive influence maximization (my first research paper!); and, last but not
least, to \textbf{Jessica Gameiro}, for her invaluable assistance with all administrative issues.

As this thesis marks the end of my long studies, I would like to thank all the professors who encouraged me during my years in Bayonne, Toulouse, and Paris. In particular, at a time when I was still hesitating to embark on a PhD, my discussions with \textbf{Pierre Alquier}, then at
ENSAE Paris, helped me see things more clearly. Furthermore, I am indebted to all members of the scientific community who contributed to the Python open-source libraries and tools that are cited and used throughout this thesis. In particular, many thanks to \textbf{Thomas Kipf} from Google Research, as my experiments often relied on his Tensorflow implementations of graph autoencoders and graph convolutional networks. Finally, like many researchers, I also owe a lot
to \textbf{Alexandra Elbakyan} and her major contributions towards making science more accessible.

On a more personal level, I would like to thank \textbf{Damien Silès} for the invaluable pieces of life advice he has been providing me since we met, and for helping me to be proud of who I am. Moreover, my life in Paris would not be the same without the never-failing support of my
close friends \textbf{Gautier Appert} and \textbf{Man Zhang}. It was inconceivable for me to write these acknowledgments without mentioning them. I am confident that our future will hold many more culinary discoveries and endless geek discussions. Of course, as this thesis deals with music, I also have a very special thought for my dear musician friends \textbf{Fabien Castillon}, \textbf{Mélissa Castillon}~and~\textbf{Kévin Hamard}.%, 

Je passe désormais de l'anglais au français, afin d'adresser un remerciement tout particulier à l'ensemble de \textbf{ma famille}, et notamment à mon père, à ma mère, à ma s\oe{}ur, à mon frère, ainsi qu'à mes quatre grands-parents. Je ne serai pas arrivé où j'en suis sans leur amour et
leur soutien inconditionnels. J'espère que cette thèse les rendra fiers. Mes parents m'ont aussi accueilli, épaulé et supporté (je sais que ça n'est pas toujours facile) le temps de la rédaction de celle-ci dans mon Pays Basque natal. Grâce à eux, j'ai pu terminer ce long projet dans les
meilleures conditions possibles. Je leur en suis reconnaissant.



I dedicate this last paragraph, perhaps the most important one, to my life partner \textbf{Jiaying~Xu}. Without her encouragement and loving support, I would never have considered starting this thesis. She accompanied me and helped me in all the steps of this long project. In recognition of her patience, attention, and benevolence throughout these years, she should have received a diploma as well. I am extremely lucky to have her by my side, and I am confident that our future is bright and full of exciting new adventures.

$$ $$

\begin{flushright}
Guillaume
\end{flushright}


==> frontmatter/dedication.tex <==
\addcontentsline{toc}{section}{Preface}


To my family.

==> frontmatter/frenchabstract.tex <==

Les graphes sont des structures omniprésentes dans de nombreux domaines de recherche, allant de l’étude des réseaux sociaux à la recommandation automatique de contenu en passant par la biologie. Cette omniprésence est due à la prolifération de données représentant les relations ou les interactions entre des entités, aussi appelées des nœuds. Dans un graphe, ces relations et interactions sont résumées sous la forme de liens, aussi appelés des arêtes, qui relient~ces~nœuds~entre~eux.  

Extraire de l'information pertinente au sujet des nœuds et des arêtes d'un graphe est essentiel pour espérer résoudre de nombreux problèmes d'apprentissage machine. Cela inclut notamment la prédiction de liens manquants entre des paires de nœuds, ainsi que la détection de communautés de nœuds, deux problèmes sur lesquels nous nous concentrons tout particulièrement au sein de cette thèse. 
Au cours des dernières décennies, diverses méthodes ont été proposées afin de résoudre de tels problèmes d'apprentissage. Alors que des approches traditionnelles proposaient de construire manuellement des indicateurs statistiques résumant les nœuds et leurs connexions, des améliorations significatives ont récemment été obtenues par des méthodes visant à directement apprendre, au travers d'un modèle, les meilleures représentations vectorielles des nœuds d'un graphe selon certains critères prédéfinis.

En particulier, les autoencodeurs de graphes (GAE) et les autoencodeurs variationnels de graphes (VGAE) se sont récemment imposés comme deux puissants groupes de méthodes permettant de construire de telles représentations vectorielles de manière non supervisée, avec des applications prometteuses à de divers problèmes d'apprentissage dont ceux cités précédemment. Au début de notre recherche, les GAE et VGAE souffraient néanmoins de plusieurs limitations majeures, que nous détaillons tout au long de cette thèse. Ces limitations entravaient l'utilisation des GAE et VGAE dans le cadre d'applications industrielles à grande échelle, par exemple liées à la recommandation musicale au sein du service de \textit{streaming} musical Deezer, où ce doctorat a été réalisé.


Dans cette thèse, nous présentons plusieurs contributions permettant d'améliorer les GAE et VGAE et de faciliter de telles utilisations. Tout d'abord, nous proposons deux stratégies permettant  de surmonter les problèmes de passage à l'échelle des GAE et VGAE, et d'entraîner ces modèles sur des graphes ayant des millions de nœuds et d'arêtes tels que ceux disponibles chez Deezer. Ces stratégies exploitent respectivement des techniques de dégénérescence de graphes et de décodage stochastique de sous-graphes.
Par ailleurs, nous présentons nos GAE et VGAE inspirés de la gravité (de l'anglais \textit{Gravity-Inspired GAE and VGAE}). Il s'agit des premières extensions de ces modèles destinées aux graphes dirigés, qui sont omniprésents dans les applications industrielles. Ces extensions obtiennent de meilleurs résultats empiriques que plusieurs alternatives populaires pour différents problèmes de prédiction de liens manquants dirigés. Nous étudions également des extensions des GAE et VGAE destinées aux graphes dynamiques, dans lesquels les nœuds et les arêtes peuvent évoluer au cours du temps.
En outre, nous démontrons que les GAE et VGAE existants, qui reposent en général sur des réseaux convolutifs de graphes (GCN) multi-couches, sont souvent inutilement complexes. Par conséquent, nous proposons de les simplifier, en ayant recours à des encodeurs linéaires. 
 Enfin, nous présentons nos GAE et VGAE informés par la modularité (de l'anglais  \textit{Modularity-Aware GAE and VGAE}), qui permettent d'améliorer la détection de communautés de nœuds, tout en préservant de bonnes performances pour la prédiction de liens manquants.


Dans la dernière partie de cette thèse, nous évaluons nos méthodes sur plusieurs graphes extraits du service de \textit{streaming} musical Deezer. Nous nous concentrons sur des problèmes de recommandation musicale à partir de graphes, souvent présentés sous la forme de problèmes de prédiction de liens manquants ou de détection de communautés de nœuds.
En particulier, nous montrons que nos méthodes permettent d'améliorer la détection de communautés d'entités musicales à recommander aux mêmes utilisateurs, mais aussi de mieux classer des artistes similaires dans un contexte de démarrage à froid (de l'anglais \textit{cold start}), et enfin de mieux modéliser la perception des genres musicaux à travers différentes cultures. 
Pour terminer, nous présentons également deux autres modèles, récemment déployés en production chez Deezer afin de recommander de la musique à des millions d'utilisateurs. Ces deux modèles permettent respectivement de personnaliser les carrousels de playlists et d'albums proposés aux utilisateurs sur la page d'accueil de Deezer et, dans un contexte de démarrage à froid, de recommander du contenu musical aux nouveaux utilisateurs du service, pour lesquels peu de données sont disponibles. Bien qu'étant moins directement liés aux GAE et VGAE, ces deux derniers projets fournissent un point de vue complémentaire sur des sujets de recommandation musicale connexes à ceux étudiés précédemment.

==> frontmatter/preface.tex <==
\addcontentsline{toc}{section}{Preface}



This PhD thesis presents research conducted from October 2018 to September 2021. It is the outcome of a scientific collaboration between the music streaming service \textbf{Deezer}, where the PhD candidate is a permanent employee in the ``Deezer Research'' team in Paris, France, and the \textbf{Laboratoire d'informatique de l'École polytechnique (LIX)}, in Palaiseau, France. This project has been entirely funded by Deezer.


==> frontmatter/symbols.tex <==
\addcontentsline{toc}{section}{List of Acronyms and Symbols}

\paragraph{Common Acronyms}
\begin{itemize}
    \item \textbf{AE}: Autoencoder;
    \item \textbf{ALS}: Alternating Least Squares;
    \item \textbf{AMI}: Adjusted Mutual Information;
    \item \textbf{AP}: Average Precision;
    \item  \textbf{APP}: Asymmetric Proximity Preserving;
    \item \textbf{ARI}: Adjusted Rand Index;
    \item \textbf{AUC}: Area Under the ROC Curve;
    %\item \textbf{BERT}: Bidirectional Encoder Representations from Transformers;
    \item \textbf{CVAE}: Collaborative Variational Autoencoder;
    \item \textbf{DEAL}: Dual-Encoder Graph Embedding with Alignment;
    \item \textbf{DVGAE}: Dirichlet Variational Graph Autoencoder;
    \item \textbf{ELBO}: Evidence Lower Bound;
    \item \textbf{GAE}: Graph Autoencoder;
    \item \textbf{GCN}: Graph Convolutional Network;
    \item \textbf{GNN}: Graph Neural Network;
    \item \textbf{HOPE}: High Order Proximity Preserved Embedding;
    \item \textbf{KL}: Kullback-Leibler;
    %\item \textbf{FT}: Language-Agnostic Sentence Representations;
    \item \textbf{LINE}: Large-Scale Information Network Embedding;
    \item \textbf{MAP}: Mean Average Precision;
    \item \textbf{MeLU}: Meta-Learned User Preference Estimator;
    \item \textbf{MGAE}: Marginalized Graph Autoencoder;
    \item \textbf{NDCG}: Normalized Discounted Cumulative Gain;
    \item \textbf{NLP}: Natural Language Processing;
    \item \textbf{NN}: Neural Network;
    \item \textbf{ReLU}: Rectified Linear Unit;
    \item \textbf{ROC}: Receiver Operating Characteristic;
    \item \textbf{SGC}: Simple Graph Convolution;
    \item \textbf{SVD}: Singular Value Decomposition;
    \item \textbf{TS}: Thompson Sampling;
    \item \textbf{UCB}: Upper Confidence Bound;
    \item \textbf{VAE}: Variational Autoencoder;
    \item \textbf{VGAE}: Variational Graph Autoencoder;
    \item \textbf{VGAECD}: Variational Graph Autoencoder for Community Detection.
    %\item \textbf{WL}: Weisfeiler-Lehman;
    %\item \textbf{XLM}: Cross-Lingual Language Model.
\end{itemize}


\paragraph{Common Linear Algebra Symbols and Operations}
For some dimension $p \in \mathbb{N}^*$, some vectors $a \in \mathbb{R}^p$ and $b \in \mathbb{R}^p$, and some square matrices $M \in \mathbb{R}^{p \times p}$ and $N \in \mathbb{R}^{p \times p}$:
\begin{itemize}
    \item $\mathbf{1}_p$: the $p$-dimensional vector containing $p$ entries all equal to 1;
    \item $a_i \in \mathbb{R}$: the $i$-th element of $a$, for some $i \in  \{1, \dots, p\}$;
    \item $M_{ij} \in \mathbb{R}$: the element at the $i$-th row and $j$-th column of $M$, for some $(i,j) \in  \{1, \dots, p\}^2$;
    \item $\|a\|_2 = \sqrt{\sum\limits_{i=1}^p a^2_i} \in \mathbb{R}^+$: the Euclidean norm of $a$;
    \item $\|a - b\|_2 = \sqrt{\sum\limits_{i=1}^p (a_i - b_i)^2} \in \mathbb{R}^+$: the Euclidean distance between $a$ and $b$;
    \item $a^T b = \sum\limits_{i=1}^p a_i b_i  \in \mathbb{R}$: the inner product between $a$ and $b$;
    \item $\text{diag}(a)  \in \mathbb{R}^{p\times p}$: the $p \times p$ diagonal matrix verifying $\text{diag}(a)_{ii} = a_i,~\forall i \in \{1,\dots,p\}$ and $\text{diag}(a)_{ij} = 0,~\forall (i,j) \in \{1,\dots,p\}^2$ with $i \neq j$;
    \item $I_p = \text{diag}(\mathbf{1}_p)$: the $p \times p$ identity matrix;
    \item $M N \in \mathbb{R}^{p \times p}$: the matrix multiplication of $M$ and $N$ ($\neq NM$ in general). It extends to $M' N' \in \mathbb{R}^{p_1 \times p_3}$, for two matrices $M' \in \mathbb{R}^{p_1 \times p_2}$ and $N' \in \mathbb{R}^{p_2 \times p_3}$ with $p_1, p_2, p_3 \in \mathbb{N}^*$;
    \item $M^T \in \mathbb{R}^{p \times p}$: the transpose of $A$, verifying: $\forall (i,j) \in \{1, \dots, p\}^2, M^T_{ij} = M_{ji}$;
    \item $M^{-1} \in \mathbb{R}^{p \times p}$: the inverse of $M$, assuming $M$ is nonsingular, i.e., $M M^{-1} = M^{-1} M~=~I_p$;
    \item $\text{Tr}(M) = \sum\limits_{i=1}^p M_{ii} \in \mathbb{R}$: the trace of $M$;
    \item $M = U \Lambda U^{-1}$, with $U \in \mathbb{R}^{p \times p}$ and $\Lambda \in \mathbb{R}^{p \times p}$: the eigendecomposition of $M$, assuming $M$ is diagonalizable. We denote by $u_i \in \mathbb{R}^p$ the eigenvector associated with an eigenvalue $\lambda_i \in \mathbb{R}$ of $M$, i.e., it verifies $M u_i = \lambda_i u_i$. Here, $\Lambda$ denotes the diagonal matrix containing the $p$ eigenvalues $\lambda_1, \dots,\lambda_p$ of $M$ in the diagonal. $U = [u_1,\dots, u_p]^T$ contains their corresponding eigenvectors $u_1,\dots,u_p$ as rows. If $U$ is orthogonal, we have: $M = U \Lambda U^{T}$;
    \item $\|M\|_F = \sqrt{\text{Tr}(M^T M)} = \sqrt{\sum\limits_{i=1}^p \sum\limits_{j=1}^p M^2_{ij}} \in \mathbb{R}^+$: the Frobenius norm of $M$;
    \item  $\|M - N\|_F = \sqrt{\sum\limits_{i=1}^p \sum\limits_{j=1}^p (M_{ij} - N_{ij})^2} \in \mathbb{R}^+$: the Frobenius distance between $M$ and $N$.
\end{itemize}

\paragraph{Common Graph Representation Learning Symbols}
\begin{itemize}
    \item $\mathcal{G} = (\mathcal{V},\mathcal{E})$: a graph composed of a node set $\mathcal{V}$ and an edge set $\mathcal{E}$;
    \item $i \in \mathcal{V}$: a node $i$ from $\mathcal{G}$;
    \item $(i,j) \in \mathcal{E}$: an edge connecting node $i$ to node $j$ in $\mathcal{G}$;
    \item $\mathcal{N}(i) \subseteq \mathcal{V}$, $\mathcal{N}_{\text{in}}(i) \subseteq \mathcal{V}$, $\mathcal{N}_{\text{out}}(i)  \subseteq \mathcal{V}$: the neighborhood, incoming neighborhood and outcoming neighborhood of a node $i \in \mathcal{V}$, respectively;
    \item $w_{ij} \in [0,1]$: the normalized weight associated with the edge $(i,j)$;
    \item $n \in \mathbb{N}^*$: the number of nodes in $\mathcal{G}$, i.e., $n= |\mathcal{V}|$;
    \item $m \in \mathbb{N}$: the number of edges in $\mathcal{G}$, i.e., $m= |\mathcal{E}|$;
    \item $f \in \mathbb{N}^*$: the dimension of feature vectors describing each node;
\item $x_i \in \mathbb{R}^f$ : the feature vector describing node $i \in \mathcal{V}$; 
\item $X \in \mathbb{R}^{n \times f}$: the node feature matrix, stacking up all $x_i$ vectors;
\item $d \in \mathbb{N}^*$: the dimension of the node embedding space;
\item $z_i \in \mathbb{R}^d$: the embedding vector of node $i \in \mathcal{V}$;
\item $Z \in \mathbb{R}^{n \times d}$: the node embedding matrix, stacking up all $z_i$ vectors;
\item $A \in [0,1]^{n \times n}$: the adjacency matrix of $\mathcal{G}$;
\item $\tilde{A} \in [0,1]^{n \times n}$: the symmetric normalization of $A$;
\item  $\tilde{A}_{\text{out}} \in [0,1]^{n \times n} $: the out-degree normalization of $A$;
\item $\hat{A} \in [0,1]^{n \times n} $: the adjacency matrix reconstructed by a GAE or VGAE model;
\item $D_{\text{in}} \in [0,n]^{n \times n}$: the in-degree matrix of $\mathcal{G}$;
\item $D_{\text{out}} \in [0,n]^{n \times n}$: the out-degree matrix of $\mathcal{G}$;
\item $D \in [0,n]^{n \times n}$: the degree matrix of $\mathcal{G}$, for an undirected graph;
\item $L_{\text{un}} \in [-1,n]^{n \times n}$: the unnormalized Laplacian matrix of $\mathcal{G}$;
\item $L_{\text{rw}} \in [-1,n]^{n \times n}$: the random-walk normalized Laplacian matrix of $\mathcal{G}$;
\item $L_{\text{sym}} \in [-1,n]^{n \times n}$: the symmetrically normalized Laplacian matrix of $\mathcal{G}$;
\item $K \in \{1, \dots, n\}$: the number of communities in $\mathcal{G}$;
\item $C_1 \subseteq \mathcal{V}, \ldots, C_K \subseteq \mathcal{V}$: a partition of $\mathcal{V}$ into $K$ communities;
\item $A_c \in \{0,1\}^{n \times K}$: the community membership matrix corresponding to the above partition;
\item $A_s \in \{0,1\}^{n \times K}$: the $s$-regular sparsification of the above matrix $A_c$;
\item $L \in \mathbb{N}^*$: the number of layers in a GNN, excluding the input layer;
\item $d_l \in \mathbb{N}^*$: the dimension of layer $l \in \{0,\dots,L\}$, with $l=0$ denoting the input layer;
\item $h^{(l)}_i \in \mathbb{R}^{d_l}$: the vectorial representation of node $i \in \mathcal{V}$ at layer $l \in \{0,\dots,L\}$; 
\item $H^{(l)}\in \mathbb{R}^{n \times d_l}$: the matrix stacking up all $h^{(l)}_i$ vectors, for $l \in \{0,\dots,L\}$;
\item $W^{(l)} \in \mathbb{R}^{d_{l} \times d_{l+1}}$: in a GCN, the weight matrix from layer $l$ to $l+1$, for $l \in \{0,\dots,L-1\}$;
\item $\sigma: \mathbb{R} \rightarrow ]0,1[$: the sigmoid activation function (the notation $]0,1[$ indicates that 0 and 1 are excluded from the set);
\item $\text{ReLU}: \mathbb{R} \rightarrow \mathbb{R}^+$: the ReLU activation function;
\item $\mathcal{L}_{\text{MODEL}}: \mathcal{I} \rightarrow  \mathbb{R}$: the loss/objective function of a model, with input elements in a set~$\mathcal{I}$;
%\item $\mathcal{N}: \mathbb{R} \rightarrow \mathbb{R}^+$: the density of a (usually multi-dimensional) Gaussian distribution. Its mean vector $\mu$ and variance matrix $\Sigma$ will often be explicitly specified (as $\mathcal{N}(\cdot|\mu, \Sigma)$);
%\item $\mathbb{E}: \mathcal{P} \rightarrow \mathbb{R}$: the expectation of a random variable defined on a probability space $\mathcal{P}$; 
%\item $\mathcal{D}_{\text{KL}}: \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}^+$: the Kullback-Leibler divergence, for two densities defined on the same support $\mathcal{X}$;
\item $\delta^{*}(\mathcal{G}) \in \{0, \dots, n\}$: the degeneracy number of $\mathcal{G}$;
\item  $\mathcal{C}_{\delta^*(\mathcal{G})} \subseteq \mathcal{C}_{\delta^*(\mathcal{G})-1} \subseteq ... \subseteq \mathcal{C}_{0} = \mathcal{V}$: the core decomposition of $\mathcal{G}$.
\end{itemize}

